AAD-LLM: Adaptive Anomaly Detection Using Large Language Models

For data-constrained, complex and dynamic industrial environments, there is a critical need for transferable and multimodal methodologies to enhance anomaly detection and therefore, prevent costs associated with system failures. Typically, traditional PdM approaches are not transferable or multimodal. This work examines the use of Large Language Models (LLMs) for anomaly detection in complex and dynamic manufacturing systems. The research aims to improve the transferability of anomaly detection models by leveraging Large Language Models (LLMs) and seeks to validate the enhanced effectiveness of the proposed approach in data-sparse industrial applications. The research also seeks to enable more collaborative decision-making between the model and plant operators by allowing for the enriching of input series data with semantics. Additionally, the research aims to address the issue of concept drift in dynamic industrial settings by integrating an adaptability mechanism. The literature review examines the latest developments in LLM time series tasks alongside associated adaptive anomaly detection methods to establish a robust theoretical framework for the proposed architecture. This paper presents a novel model framework (AAD-LLM) that doesn't require any training or finetuning on the dataset it is applied to and is multimodal. Results suggest that anomaly detection can be converted into a "language" task to deliver effective, context-aware detection in data-constrained industrial applications. This work, therefore, contributes significantly to advancements in anomaly detection methodologies.

==> component_subject_sections/Discussion/discussion.tex <==
discussion

==> component_subject_sections/Limitation/limitation.tex <==
limitation

==> component_subject_sections/Method-Proposal-Main_Analysis/main_thing.tex <==
\hl{extensive work will be done on this section, the below is little more than a note to authors.}

\subsection{Hypothesis}
This project seeks to test the hypothesis that a mildly extended version of Time-LLM\cite{Time_LLM} can supply Transferable PdM capabilities within a closely related set of mechanical systems. 

\subsection{Datasets}
Our use case would concern one or more of the following:
\begin{itemize}
    \item A dataset provided by the company Ms. Gilbert works for. It would be time series data from a number of sensors monitoring the condition of components of a plastic film production line. As a real-world use case we can expect faults to be extant but rare relative to healthy data.
    \item Either of the C-MAPSS datasets, the second is probably less published on.
    \item The FEMTO dataset.
    \item The CAVS MFS data that Dr. Amirlatifi has been working with. Note that this isn't a true RTF dataset and so would require a different partitioning scheme. It can have nominal and anomalous samples though, which means it could be used.
\end{itemize}
Selecting any one dataset, it would be partitioned according to a scheme shared with the diffusion-project.

\subsection{Shared Partitioning Scheme}
    Under the assumption that our dataset consists of $n$ complete run-to-failure (RtF) records with $d$ features over time, let:
    \begin{itemize}
        \item $o$ be the offset backwards in time from the end-of-life (EoL).
        \item $k$ be the number of complete RtFs in the ``available" partition $A$. These RtFs are ``complete", and others are ``incomplete".
        \item $\gamma$ modify the amount of nominal data from the $n-k$ that can be in $A$.
        \item $M$, the ``missing" partition, be all data not in $A$.
    \end{itemize}

    There are $\binom{n}{k}$ gross partitions of the data. Variation of $\gamma$ within each partition produces even more partitions-proper.
    $o$ here is a number of time-steps, and each time-step within that window backwards from the EoL of an RtF is defined as some amount of anomalous. $\gamma$ might be a number of time steps, but could also be a percentage. In any case, the number of nominal time-steps placed in $A$ from incomplete RtFs cannot exceed those which actually exist, so a high time-step $\gamma$ might be truncated for shorter RtFs.

    Because the LLM-reprogramming project seeks to explore transferability, it may have a $\gamma$ of 0, this is unadvised for the diffusion project. For the LLM-project more than the other, the $\frac{A}{M}$ ratio, a function of $k$, can be explored to test transferability, which is a core part of exploring that project's hypothesis.

    A series of partitions are used to explore each project's hypothesis, similar to standard k-fold repetition. 

    While this scheme is shared between the projects, the values of the hyperparameters do not need to be (nor do the datasets, though this would be convenient).

\subsection{Anomaly Detection and the Current Time-LLM operation}
Anomaly detection aligns well with the lab's other PdM work. The Time-LLM model currently only implements varied range forecasting, so modification \emph{would} be necessary. Having examined the code, this modification seems quite doable in the anticipated timeline of the project, an \emph{abstract} description of the current model's pipeline follows:
\begin{enumerate}
    \item Assume a trained model.
    \item A $d$-variate time series segment $s$ of length $l$ is selected as input. $s \in \mathbf{R}^{d \times l}$ where $d$ is the number of features native to the time series.
    \item $s$ is ``patched" with a window of size $w$ using a stride of $a$, producing $p$ patches. The input is now $\in \mathbf{R}^{p \times d \times w}$. This deserves some explanation:
    \begin{displayquote}
        $w$ will be used as an analog to a word embedding. NLP sequences are semantically dense. each word has a lot of ``meaning" even before that meaning is modified by other words. This is reflected in the high dimensionality most word embeddings use to capture meaning. Sentences are also short relative to many signals. Time-series are often the inverse: semantically shallow series of great length. The most meaningful part of a time-series is usually the way a signal moves over time, not the signal at any given time. Patching, introduced in \cite{Patching}, is a way of moving between the time-domain and what we will analogize as the ``semantic" domain. For a given window over a uni-variate time series, it's ``embedding" is a linear projection of its transpose, sometimes followed by a nonlinear activation function.
    \end{displayquote}
    \item The $d$ covariates are hidden from eachother in the batch dimension, meaning that instead of $b$ batch elements, each with $d$ features over time, there are now $b \times d$ batch elements with one feature over time each. This means that the individual features of each batch element are processed in isolation, which is worth noting because it differentiates this process from others where they are allowed to influence one another during the forward pass.
    \item The $p$ sequential size $w$ patches are now projected up to some operating dimension and treated as embeddings.
    \item Now the ``reprogramming" step.
    \begin{displayquote}
        For the frozen LLM in the middle of the model, there is a set of word embeddings $E$ that it was trained using. Let a text prototype $f$ be a linear combination of the $n$ word embeddings in $ E = \{e_{1}, e_{2}, ..., e_{n}\}$. With a set of prototypes $F$, and a self attention mechanism (key-query-value dot product softmax attention), the set of all patches generated from a time-series are used as the query source with the text prototypes used as the keys and value sources. This ``translates" the time series into the language domain. This is similar to encoder-decoder attention and ``cross" attention \cite{Cross_attention_origin}.   
    \end{displayquote}
    \item A prompt, used to instruct the LLM, is created (this step is automated). The prompt also reports some statistical derivatives of $s$, and the translation of $s$. \emph{This} is what is given to the LLM.
    \item The frozen LLM processes the input sequence, and the output sequence is truncated from the end such that only the last $p$ elements are kept. These correspond to $s$, the cut content refers to the prompt. If inference time is a problem, a quantized model can be used. Most LLMs available are compatible with the methodology design.
    \item For forecasting, the output is flattened and passed through a single, but quite large, linear layer to output the forecaster values. The current work might do something different.
\end{enumerate}

Most of our modifications will concern the prompt, the statistical derivatives, and the output pipeline. While these modifications \emph{will} be part of the work as research, we want to \emph{minimize} the amount of engineering and invention. Finding good targets for the output pipeline will be part of the lit review, even if only to verify that there isn't a best practice, in which case we must devise a \emph{reasonable and consistent} answer. If we do not substantially change the output pipeline, a varied prompting scheme can be a potential publishable contribution, alongside the novelty of the anomaly detection application. Common anomaly detection trains a model to accept an instance of data, such as $s$, and assign it to the class of anomalous or nominal behavior. An alternative this project could pursue, which might be more amenable to transfer learning, is to supply two data instances $C$ and $Q$ where $C$ is the ``comparator" and $Q$ is the ``query". In this setup, the model is trained to evaluate the normality of the instance $Q$ given an assumed nominal instance $C$. In this training scheme the model is tuned to compare samples, rather than assess a sample singularly. To analogize this to an image classification task: Classic anom.-det. is like labeling images of animals, where as this comparison scheme is like rating the similarity of the class of two pictures.

In each case, the hypothesis being tested is the same: Can the proof of concept model be tuned on a subset of the data and perform the PdM task on the unseen partition.

\subsection{Likely Questions}
\begin{enumerate}
    \item Why should an LLM be able to forecast, or commit any time-series task?
    \begin{displayquote}
        While a \emph{good} question, it is important to remember that answering it is \emph{secondary}, at most, to \emph{this} project at \emph{this} stage. This summer concerns application more than theory. That said, the text-prototyping, and ($s$ $\rightarrow$ $\approx $ Nat. Lang. $\rightarrow \{\text{class, regression-value}\}$) pipeline seem to do the following: While usually lossy, a time series can be described in natural language. Simple sinusoids can be perfectly translated becasue they have reserved names and we can number the frequency. But supposing we couldn't. A translation might be: ``Smoothly oscillating at a fixed frequency $x$". A crypto-currency rise and fall could be described with such terms as ``jagged", ``sudden", and ``crash". As is usually the case in ML, outside of explainability, we often concern ourselves with the possibility of learning useful features and functions, not exactly what features and functions \emph{are} learned. In the case of the text-prototypes, they are a learned parameter of the pre-LLM translation module. In the paper introducing Time-LLM, the authors discovered that words relevant to describing time-series had a much greater coefficient in the linear combinations that constitute the prototypes. This suggests that the projection which creates the prototypes learns which words best translate the time-series, and that these words minimize the model's loss. After translation, the extensive question-answering and next word prediction capacities of the LLM do \textbf{something} useful. It is, again, not the aim of this project to interrogate that \textbf{something}. It is likely that the robust natural language feature extraction capacities of the LLM provide the output translation layer with a substantially easier task than it would have otherwise.

        Outside of this particular application, LLMs are not my domain of expertise. As I understand it, they are only able to usefully ``reason" (and that word is generously used here) on subject matter they are either parametrically familiar with (which was robustly represented in their training data) or with which they are supplied using methods such as retrieval augmented generation \cite{RAG}. Without RAG, or a use-case specific training set, I would not expect an LLM to be usefully informed about most PdM use-cases, but its NLP capabilities might make for plausible sounding responses. We must be very careful in how we evaluate such responses.

        Any confidence I have in the domain transferability of reprogramming approaches is conditionally based on their reported performance \cite{LLM_reprogramming, Time_LLM, LLM_in_TS, LLM_zero_shot_TS}, and the notion of the LLM as a feature extractor, more than a question answering system.
    \end{displayquote}
    \item Why should we pursue this $C$ $Q$ comparison over more traditional input configurations?
    \begin{displayquote}
        Perhaps we shouldn't, that is what this early stage of critique and investigation is for. A compare-contrast input style will train the model to extract features from $C$, and treat them as a baseline against which the features of $Q$ can be compared. This could be a more use-case agnostic approach because the model will be less incentivized to memorize the nominal and anomalous features of a particular use-case, and instead learn a more generic feature extraction and comparison function. With sufficient time, the model can be tested on both schemes since they would only require minor edits to the input pipeline and prompt.
    \end{displayquote}
    \item How would the $C$ $Q$ input be structured?
    \begin{displayquote}
        This is something we can look into, but we should set a default. Based on the prompt-as-prefix style used in the Time-LLM paper, it seems that we can use the prompt as a kind of conditioning signal. Provided we set a consistent pattern, the prompt can inform the model about the rest of the input, and modify its process. We might try one of two arrangements.
        \begin{enumerate}
            \item $<$use-case context description. Ex: Here are two time-series from an air-conditioner$>$ $<$task prompt. Ex: The first series is normal data. Is the second normal or abnormal by comparison? They are separated by padding with 0s.$>$ (note that we would need to pad with 0s) $<$TS1 statistics$>$ $<$TS1$>$ $<$padding$>$ $<$TS2 statistics$>$ $<$TS2$>$
            \item $<$use-case context description. Ex: We have two time-series from a refrigeration unit.$>$ $<$task prompt A: given that$>$ $<$TS1 statistics$>$ $<$TS1$>$ $<$task prompt B: is normal, is $>$ $<$TS2 statistics$>$ $<$TS2$>$ $<$task prompt C: abnormal by comparison?$>$
        \end{enumerate}
        These prompts might be enriched by some number of provided examples, where we include some number of ($C$, $Q$) pairs along with the expected output. These are followed by our target ($C$, $Q$) pair. This kind of example providing is apparently a common method from prompt engineering, which will be a concern of this project, but will be mostly left to future work after a workable format has been selected. Investigation would take place in the realm of feature engineering.
        
        Iteration of the prompt/input format will be less work relative to editing the output pipeline, since most of the implementation has been done by the Time-LLM team. \href{https://www.promptingguide.ai/models/mistral-7b}{This} shows examples of prompt architecture.
    \end{displayquote}
    \item Why are the covariates hidden from one another until the output pipeline?
    \begin{displayquote}
        This seems to be because the translation step operates only on univariate time-series, but this only pushes the question back: Why would it do this? It seems like this is an accommodation for the LLM. Language is ``univeriate" in that we do not process more than one sentence in parallel. True, the concepts communicated are often dense, and the mind does a lot of parallel processing, but language itself is still linear and singular, and LLMs process these linear, singular sequences. Fortunately the output pipeline is not limited to univariate functions, and can learn functions which interact the covariates.
    \end{displayquote}
\end{enumerate}

==> component_subject_sections/Notes/Notes.tex <==
Current action items:
\begin{itemize}
    \item action item 1
    \item \hl{use highlighting to leave notes to authors, including self, in the text}
    \item \hl{Remember the narrative.}
    \item When reviewing one another's work, give in-text examples and provide heuristics for how to write something better, try to avoid $\approx$ ``make it better" statements.
\end{itemize}

==> component_subject_sections/Recommendations-Future_Work/rec_fw.tex <==
recomendations and future work
